CCAligned: A Massive Collection of Cross-Lingual Web-Document Pairs

Cross-lingual document alignment aims to identify pairs of documents in two distinct languages that are of comparable content or translations of each other. In this paper, we exploit the signals embedded in URLs to label web documents at scale with an average precision of 94.5% across different language pairs. We mine sixty-eight snapshots of the Common Crawl corpus and identify web document pairs that are translations of each other. We release a new web dataset consisting of over 392 million URL pairs from Common Crawl covering documents in 8144 language pairs of which 137 pairs include English. In addition to curating this massive dataset, we introduce baseline methods that leverage cross-lingual representations to identify aligned documents based on their textual content. Finally, we demonstrate the value of this parallel documents dataset through a downstream task of mining parallel sentences and measuring the quality of machine translations from models trained on this mined data. Our objective in releasing this dataset is to foster new research in cross-lingual NLP across a variety of low, medium, and high-resource languages.

==> emnlp/data.tex <==
target_dialect	_col1
ss_SZ	6
ff_NG	18
ns_ZA	48
ln_CD	48
om_KE	102
lg_UG	123
tn_BW	166
zu_ZA	249
wo_SN	529
ta_IN_rom	655
as_IN	782
jv_ID	1025
cb_IQ	1154
te_IN_rom	1210
or_IN	1369
bn_IN_rom	1468
ur_PK_rom	1827
br_FR	2366
xh_ZA	2762
cx_PH	3038
ig_NG	6105
ar_AR_rom	7428
su_ID	7484
yo_NG	7583
mg_MG	7881
bs_BA	9461
ha_NG	9473
ps_AF	10340
so_SO	13948
my_MM	14231
lo_LA	14310
am_ET	14942
pa_IN	15728
gu_IN	18879
te_IN	19257
mr_IN	21079
kn_IN	21541
mn_MN	24062
km_KH	26089
si_LK	27303
hi_IN_rom	27633
ml_IN	29134
ne_NP	30263
ht_HT	32464
kk_KZ	36058
be_BY	38185
ta_IN	41838
sw_KE	42012
af_ZA	43384
tl_XX	50197
ur_PK	51968
sq_AL	57955
sr_RS	61525
bn_IN	62773
is_IS	64385
hy_AM	66580
ka_GE	71410
cy_GB	87618
mk_MK	94312
az_AZ	97998
et_EE	159655
lv_LV	169112
sl_SI	174434
ms_MY	176926
lt_LT	183068
fa_IR	206269
hi_IN	232691
he_IL	276248
uk_UA	298571
hr_HR	316686
sk_SK	328341
vi_VN	345366
ca_ES	353488
bg_BG	441444
no_XX	447538
id_ID	449228
th_TH	477723
fi_FI	487585
ro_RO	511216
hu_HU	522741
da_DK	546521
zh_TW	623631
cs_CZ	640649
sv_SE	720724
ko_KR	723251
el_GR	771943
tr_TR	949488
ar_AR	1047667
pl_PL	1233121
zh_CN	1594290
ja_XX	1638758
pt_XX	1728374
nl_XX	2017971
it_IT	2988307
ru_RU	3882330
es_XX	4369596
fr_XX	5586773
de_DE	5690159
